Bright but slow - Type II supernovae from OGLE-IV - Implications for magnitude limited surveys

We study a sample of 11 Type II supernovae (SNe) discovered by the OGLE-IV survey. All objects have well sampled I-band light curves, and at least one spectrum. We find that 2 or 3 of the 11 SNe have a declining light curve, and spectra consistent with other SNe II-L, while the rest have plateaus that can be as short as 70d, unlike the 100d typically found in nearby galaxies. The OGLE SNe are also brighter, and show that magnitude limited surveys find SNe that are different than usually found in nearby galaxies. We discuss this sample in the context of understanding Type II SNe as a class and their suggested use as standard candles.

==> data_Kcorrected_restframe.tex <==
\hline
\hline
SN name & rest-frame time & $I$ & $\Delta_I$ \\
\hline
OGLE-2014-SN-018 & 1.47270 & 19.438 & 0.083 \\
OGLE-2014-SN-018 & 5.37956 & 18.653 & 0.022 \\
OGLE-2014-SN-018 & 8.25974 & 18.496 & 0.016 \\
OGLE-2014-SN-018 & 12.12427 & 18.496 & 0.025 \\
OGLE-2014-SN-018 & 25.70538 & 18.457 & 0.018 \\
OGLE-2014-SN-018 & 35.29636 & 18.371 & 0.017 \\
OGLE-2014-SN-018 & 39.20328 & 18.338 & 0.018 \\
OGLE-2014-SN-018 & 41.15068 & 18.345 & 0.018 \\
OGLE-2014-SN-018 & 42.08987 & 18.339 & 0.024 \\
OGLE-2014-SN-018 & 43.06376 & 18.455 & 0.029 \\
OGLE-2014-SN-018 & 44.01478 & 18.384 & 0.022 \\
OGLE-2014-SN-018 & 45.95610 & 18.341 & 0.019 \\
OGLE-2014-SN-018 & 88.60024 & 18.540 & 0.041 \\
OGLE-2014-SN-018 & 100.24717 & 19.107 & 0.065 \\
OGLE-2014-SN-018 & 182.25189 & 20.740 & 0.167 \\
\hline
OGLE-2014-SN-009 & 1.44567 & 19.641 & 0.100 \\
OGLE-2014-SN-009 & 3.36477 & 19.482 & 0.079 \\
OGLE-2014-SN-009 & 4.30878 & 19.425 & 0.065 \\
OGLE-2014-SN-009 & 6.19501 & 19.202 & 0.049 \\
OGLE-2014-SN-009 & 9.03278 & 19.169 & 0.057 \\
OGLE-2014-SN-009 & 13.74580 & 19.185 & 0.073 \\
OGLE-2014-SN-009 & 17.52362 & 19.335 & 0.081 \\
OGLE-2014-SN-009 & 19.41935 & 19.295 & 0.061 \\
OGLE-2014-SN-009 & 22.25030 & 19.471 & 0.069 \\
OGLE-2014-SN-009 & 24.97752 & 19.470 & 0.096 \\
OGLE-2014-SN-009 & 27.88726 & 19.474 & 0.073 \\
OGLE-2014-SN-009 & 30.73833 & 19.542 & 0.080 \\
OGLE-2014-SN-009 & 33.58595 & 19.642 & 0.077 \\
OGLE-2014-SN-009 & 37.36605 & 19.530 & 0.076 \\
OGLE-2014-SN-009 & 41.15482 & 19.977 & 0.194 \\
OGLE-2014-SN-009 & 43.94476 & 19.693 & 0.102 \\
OGLE-2014-SN-009 & 47.73940 & 19.440 & 0.074 \\
OGLE-2014-SN-009 & 50.58169 & 19.914 & 0.099 \\
OGLE-2014-SN-009 & 51.49896 & 19.853 & 0.103 \\
OGLE-2014-SN-009 & 53.39837 & 19.556 & 0.095 \\
OGLE-2014-SN-009 & 54.31442 & 19.705 & 0.149 \\
OGLE-2014-SN-009 & 55.26433 & 19.775 & 0.138 \\
OGLE-2014-SN-009 & 56.18991 & 19.813 & 0.154 \\
OGLE-2014-SN-009 & 58.08340 & 19.723 & 0.112 \\
OGLE-2014-SN-009 & 61.87902 & 20.261 & 0.210 \\
OGLE-2014-SN-009 & 67.53732 & 20.071 & 0.160 \\
OGLE-2014-SN-009 & 71.30738 & 19.643 & 0.105 \\
OGLE-2014-SN-009 & 76.99472 & 20.061 & 0.131 \\
OGLE-2014-SN-009 & 79.83370 & 20.583 & 0.268 \\
OGLE-2014-SN-009 & 82.64448 & 20.319 & 0.204 \\
OGLE-2014-SN-009 & 99.68354 & 20.139 & 0.243 \\
OGLE-2014-SN-009 & 103.46829 & 21.066 & 0.607 \\
\hline
OGLE-2014-SN-004 & 2.39640 & 18.791 & 0.040 \\
OGLE-2014-SN-004 & 8.19841 & 18.576 & 0.027 \\
OGLE-2014-SN-004 & 8.21513 & 18.589 & 0.026 \\
OGLE-2014-SN-004 & 13.06174 & 18.724 & 0.049 \\
OGLE-2014-SN-004 & 18.87283 & 18.707 & 0.025 \\
OGLE-2014-SN-004 & 31.43431 & 18.754 & 0.028 \\
OGLE-2014-SN-004 & 35.31413 & 18.736 & 0.030 \\
OGLE-2014-SN-004 & 39.18022 & 18.865 & 0.036 \\
OGLE-2014-SN-004 & 43.09297 & 18.671 & 0.043 \\
OGLE-2014-SN-004 & 47.80222 & 18.772 & 0.034 \\
OGLE-2014-SN-004 & 51.74737 & 18.751 & 0.045 \\
OGLE-2014-SN-004 & 73.09946 & 18.962 & 0.041 \\
OGLE-2014-SN-004 & 79.86101 & 19.106 & 0.048 \\
OGLE-2014-SN-004 & 80.84213 & 19.130 & 0.050 \\
OGLE-2014-SN-004 & 81.80841 & 19.155 & 0.053 \\
OGLE-2014-SN-004 & 82.74754 & 19.028 & 0.059 \\
OGLE-2014-SN-004 & 83.72148 & 19.084 & 0.076 \\
OGLE-2014-SN-004 & 86.59976 & 19.416 & 0.067 \\
OGLE-2014-SN-004 & 88.53817 & 19.667 & 0.080 \\
OGLE-2014-SN-004 & 89.56543 & 19.612 & 0.084 \\
OGLE-2014-SN-004 & 90.48247 & 19.791 & 0.116 \\
OGLE-2014-SN-004 & 91.44051 & 19.928 & 0.137 \\
OGLE-2014-SN-004 & 95.32384 & 21.622 & 0.646 \\
OGLE-2014-SN-004 & 96.28737 & 20.526 & 0.246 \\
OGLE-2014-SN-004 & 98.23152 & 20.829 & 0.293 \\
\hline
OGLE-2013-SN-144 & 5.80113 & 18.574 & 0.020 \\
OGLE-2013-SN-144 & 11.58117 & 18.840 & 0.025 \\
OGLE-2013-SN-144 & 22.19751 & 18.898 & 0.018 \\
OGLE-2013-SN-144 & 25.11277 & 18.907 & 0.035 \\
OGLE-2013-SN-144 & 31.80518 & 19.010 & 0.025 \\
OGLE-2013-SN-144 & 38.52197 & 18.969 & 0.042 \\
OGLE-2013-SN-144 & 52.91353 & 19.145 & 0.028 \\
OGLE-2013-SN-144 & 57.67412 & 19.125 & 0.032 \\
OGLE-2013-SN-144 & 61.48253 & 19.226 & 0.040 \\
OGLE-2013-SN-144 & 66.34335 & 19.174 & 0.055 \\
OGLE-2013-SN-144 & 71.10378 & 19.420 & 0.042 \\
OGLE-2013-SN-144 & 74.92385 & 19.701 & 0.063 \\
OGLE-2013-SN-144 & 82.61658 & 19.805 & 0.054 \\
OGLE-2013-SN-144 & 102.75152 & 20.408 & 0.117 \\
OGLE-2013-SN-144 & 104.68021 & 21.229 & 0.273 \\
OGLE-2013-SN-144 & 105.61032 & 20.054 & 0.117 \\
OGLE-2013-SN-144 & 106.57486 & 20.965 & 0.287 \\
OGLE-2013-SN-144 & 109.42757 & 20.796 & 0.170 \\
\hline
OGLE-2013-SN-135 & 1.91149 & 19.858 & 0.083 \\
OGLE-2013-SN-135 & 12.27762 & 19.088 & 0.053 \\
OGLE-2013-SN-135 & 15.09596 & 18.893 & 0.040 \\
OGLE-2013-SN-135 & 17.00328 & 18.855 & 0.036 \\
OGLE-2013-SN-135 & 18.89521 & 19.076 & 0.056 \\
OGLE-2013-SN-135 & 22.67828 & 19.047 & 0.055 \\
OGLE-2013-SN-135 & 24.56009 & 18.968 & 0.045 \\
OGLE-2013-SN-135 & 27.43542 & 19.047 & 0.051 \\
OGLE-2013-SN-135 & 29.27276 & 19.101 & 0.048 \\
OGLE-2013-SN-135 & 32.12299 & 19.000 & 0.041 \\
OGLE-2013-SN-135 & 33.98376 & 19.055 & 0.040 \\
OGLE-2013-SN-135 & 35.91667 & 19.133 & 0.047 \\
OGLE-2013-SN-135 & 36.84544 & 19.096 & 0.051 \\
OGLE-2013-SN-135 & 39.69447 & 19.060 & 0.042 \\
OGLE-2013-SN-135 & 41.62356 & 18.941 & 0.038 \\
OGLE-2013-SN-135 & 44.45088 & 19.047 & 0.057 \\
OGLE-2013-SN-135 & 46.30845 & 18.924 & 0.047 \\
OGLE-2013-SN-135 & 49.13177 & 18.906 & 0.071 \\
OGLE-2013-SN-135 & 51.96054 & 19.062 & 0.083 \\
OGLE-2013-SN-135 & 53.87607 & 18.891 & 0.040 \\
OGLE-2013-SN-135 & 55.76420 & 19.053 & 0.036 \\
OGLE-2013-SN-135 & 63.35823 & 19.172 & 0.050 \\
OGLE-2013-SN-135 & 65.21683 & 19.117 & 0.048 \\
OGLE-2013-SN-135 & 67.06089 & 20.296 & 0.167 \\
OGLE-2013-SN-135 & 69.94284 & 19.119 & 0.053 \\
OGLE-2013-SN-135 & 71.78838 & 19.151 & 0.062 \\
OGLE-2013-SN-135 & 73.75751 & 18.983 & 0.048 \\
OGLE-2013-SN-135 & 76.52077 & 19.175 & 0.065 \\
OGLE-2013-SN-135 & 79.40039 & 18.933 & 0.057 \\
OGLE-2013-SN-135 & 81.30197 & 19.154 & 0.057 \\
OGLE-2013-SN-135 & 84.10382 & 19.305 & 0.059 \\
OGLE-2013-SN-135 & 86.02161 & 19.067 & 0.053 \\
OGLE-2013-SN-135 & 88.80966 & 19.307 & 0.094 \\
OGLE-2013-SN-135 & 94.50532 & 19.117 & 0.063 \\
OGLE-2013-SN-135 & 100.21457 & 19.400 & 0.069 \\
OGLE-2013-SN-135 & 102.05352 & 19.622 & 0.103 \\
OGLE-2013-SN-135 & 104.91325 & 19.723 & 0.146 \\
OGLE-2013-SN-135 & 107.72573 & 19.479 & 0.102 \\
OGLE-2013-SN-135 & 111.50316 & 19.638 & 0.088 \\
OGLE-2013-SN-135 & 115.27336 & 19.870 & 0.156 \\
OGLE-2013-SN-135 & 117.15767 & 20.407 & 0.264 \\
\hline
OGLE-2013-SN-048 & 1.44791 & 21.097 & 0.221 \\
OGLE-2013-SN-048 & 7.07493 & 20.144 & 0.164 \\
OGLE-2013-SN-048 & 8.95510 & 20.226 & 0.138 \\
OGLE-2013-SN-048 & 18.34028 & 19.772 & 0.078 \\
OGLE-2013-SN-048 & 24.93427 & 19.739 & 0.051 \\
OGLE-2013-SN-048 & 28.64130 & 19.856 & 0.064 \\
OGLE-2013-SN-048 & 31.47023 & 19.712 & 0.070 \\
OGLE-2013-SN-048 & 34.30848 & 19.961 & 0.131 \\
OGLE-2013-SN-048 & 40.96164 & 19.833 & 0.081 \\
OGLE-2013-SN-048 & 42.90312 & 19.718 & 0.059 \\
OGLE-2013-SN-048 & 51.35433 & 19.740 & 0.063 \\
OGLE-2013-SN-048 & 54.12135 & 19.708 & 0.049 \\
OGLE-2013-SN-048 & 55.97087 & 19.643 & 0.052 \\
OGLE-2013-SN-048 & 59.68459 & 19.491 & 0.099 \\
OGLE-2013-SN-048 & 62.54977 & 19.620 & 0.087 \\
OGLE-2013-SN-048 & 66.29807 & 19.771 & 0.071 \\
OGLE-2013-SN-048 & 69.16329 & 19.807 & 0.059 \\
OGLE-2013-SN-048 & 71.99083 & 19.700 & 0.050 \\
OGLE-2013-SN-048 & 77.62735 & 19.866 & 0.071 \\
OGLE-2013-SN-048 & 82.37164 & 19.856 & 0.059 \\
OGLE-2013-SN-048 & 87.06592 & 19.916 & 0.101 \\
OGLE-2013-SN-048 & 90.85140 & 20.154 & 0.129 \\
OGLE-2013-SN-048 & 95.48343 & 19.980 & 0.122 \\
OGLE-2013-SN-048 & 100.17403 & 19.935 & 0.080 \\
OGLE-2013-SN-048 & 107.76039 & 19.975 & 0.096 \\
OGLE-2013-SN-048 & 113.39496 & 20.532 & 0.182 \\
OGLE-2013-SN-048 & 118.17269 & 20.676 & 0.216 \\
OGLE-2013-SN-048 & 121.88340 & 20.566 & 0.162 \\
OGLE-2013-SN-048 & 136.03325 & 21.491 & 0.453 \\
OGLE-2013-SN-048 & 140.75650 & 21.574 & 0.446 \\
\hline
OGLE-2013-SN-047 & 4.26540 & 18.383 & 0.017 \\
OGLE-2013-SN-047 & 9.91606 & 18.274 & 0.015 \\
OGLE-2013-SN-047 & 12.81192 & 18.320 & 0.017 \\
OGLE-2013-SN-047 & 15.43081 & 18.403 & 0.019 \\
OGLE-2013-SN-047 & 18.35889 & 18.426 & 0.023 \\
OGLE-2013-SN-047 & 25.00560 & 18.634 & 0.025 \\
OGLE-2013-SN-047 & 27.85091 & 18.687 & 0.022 \\
OGLE-2013-SN-047 & 31.57273 & 18.771 & 0.028 \\
OGLE-2013-SN-047 & 39.04681 & 18.839 & 0.022 \\
OGLE-2013-SN-047 & 40.84033 & 18.922 & 0.033 \\
OGLE-2013-SN-047 & 45.76792 & 18.802 & 0.052 \\
OGLE-2013-SN-047 & 50.40425 & 18.904 & 0.028 \\
OGLE-2013-SN-047 & 53.20058 & 19.044 & 0.028 \\
OGLE-2013-SN-047 & 56.00503 & 19.003 & 0.027 \\
OGLE-2013-SN-047 & 59.77665 & 19.054 & 0.027 \\
OGLE-2013-SN-047 & 63.53497 & 19.124 & 0.030 \\
OGLE-2013-SN-047 & 68.22987 & 19.224 & 0.037 \\
OGLE-2013-SN-047 & 72.94510 & 19.193 & 0.040 \\
OGLE-2013-SN-047 & 75.79372 & 19.383 & 0.077 \\
OGLE-2013-SN-047 & 80.51809 & 19.718 & 0.077 \\
OGLE-2013-SN-047 & 82.41249 & 20.033 & 0.075 \\
OGLE-2013-SN-047 & 86.16823 & 20.575 & 0.185 \\
OGLE-2013-SN-047 & 91.72920 & 20.373 & 0.136 \\
OGLE-2013-SN-047 & 97.39075 & 20.419 & 0.123 \\
OGLE-2013-SN-047 & 100.25228 & 20.363 & 0.150 \\
OGLE-2013-SN-047 & 103.05296 & 21.194 & 0.372 \\
OGLE-2013-SN-047 & 108.80075 & 20.850 & 0.197 \\
OGLE-2013-SN-047 & 112.52144 & 20.688 & 0.168 \\
OGLE-2013-SN-047 & 113.44371 & 20.625 & 0.188 \\
OGLE-2013-SN-047 & 118.15652 & 21.115 & 0.326 \\
OGLE-2013-SN-047 & 119.10401 & 20.958 & 0.196 \\
OGLE-2013-SN-047 & 124.76485 & 20.978 & 0.305 \\
OGLE-2013-SN-047 & 131.37230 & 21.286 & 0.430 \\
OGLE-2013-SN-047 & 137.06185 & 21.499 & 0.361 \\
OGLE-2013-SN-047 & 143.61583 & 21.301 & 0.466 \\
OGLE-2013-SN-047 & 150.26151 & 21.255 & 0.282 \\
\hline
OGLE-2013-SN-046 & 1.85262 & 19.966 & 0.071 \\
OGLE-2013-SN-046 & 7.51920 & 19.617 & 0.131 \\
OGLE-2013-SN-046 & 8.43522 & 19.607 & 0.064 \\
OGLE-2013-SN-046 & 17.68373 & 19.808 & 0.059 \\
OGLE-2013-SN-046 & 23.27385 & 19.680 & 0.049 \\
OGLE-2013-SN-046 & 26.12094 & 19.802 & 0.091 \\
OGLE-2013-SN-046 & 29.75652 & 19.779 & 0.064 \\
OGLE-2013-SN-046 & 32.63357 & 19.834 & 0.074 \\
OGLE-2013-SN-046 & 38.25618 & 19.740 & 0.060 \\
OGLE-2013-SN-046 & 41.04553 & 19.728 & 0.047 \\
OGLE-2013-SN-046 & 46.72279 & 19.957 & 0.067 \\
OGLE-2013-SN-046 & 52.21227 & 19.716 & 0.039 \\
OGLE-2013-SN-046 & 54.03137 & 19.798 & 0.067 \\
OGLE-2013-SN-046 & 74.59705 & 20.005 & 0.053 \\
OGLE-2013-SN-046 & 78.34083 & 20.166 & 0.066 \\
OGLE-2013-SN-046 & 82.95838 & 20.154 & 0.077 \\
OGLE-2013-SN-046 & 93.24432 & 20.761 & 0.182 \\
OGLE-2013-SN-046 & 103.46489 & 20.780 & 0.150 \\
OGLE-2013-SN-046 & 105.31896 & 21.038 & 0.184 \\
OGLE-2013-SN-046 & 106.22566 & 20.875 & 0.188 \\
OGLE-2013-SN-046 & 108.17921 & 21.589 & 0.388 \\
OGLE-2013-SN-046 & 112.79707 & 20.927 & 0.226 \\
OGLE-2013-SN-046 & 115.60819 & 21.714 & 0.485 \\
OGLE-2013-SN-046 & 123.98885 & 21.592 & 0.279 \\
\hline
OGLE-2013-SN-045 & 2.23984 & 20.224 & 0.059 \\
OGLE-2013-SN-045 & 6.78407 & 20.404 & 0.097 \\
OGLE-2013-SN-045 & 10.28276 & 20.403 & 0.191 \\
OGLE-2013-SN-045 & 15.85615 & 20.144 & 0.112 \\
OGLE-2013-SN-045 & 24.01938 & 20.045 & 0.060 \\
OGLE-2013-SN-045 & 29.46456 & 20.026 & 0.058 \\
OGLE-2013-SN-045 & 32.25512 & 20.137 & 0.067 \\
OGLE-2013-SN-045 & 34.77878 & 20.139 & 0.075 \\
OGLE-2013-SN-045 & 37.60038 & 20.241 & 0.107 \\
OGLE-2013-SN-045 & 44.00540 & 20.175 & 0.084 \\
OGLE-2013-SN-045 & 46.74724 & 20.190 & 0.070 \\
OGLE-2013-SN-045 & 50.33372 & 20.409 & 0.108 \\
OGLE-2013-SN-045 & 57.53602 & 20.561 & 0.093 \\
OGLE-2013-SN-045 & 59.26432 & 20.251 & 0.096 \\
OGLE-2013-SN-045 & 64.01272 & 20.386 & 0.203 \\
OGLE-2013-SN-045 & 68.48045 & 20.220 & 0.080 \\
OGLE-2013-SN-045 & 71.17511 & 20.423 & 0.083 \\
OGLE-2013-SN-045 & 73.87757 & 20.346 & 0.076 \\
OGLE-2013-SN-045 & 77.51205 & 20.561 & 0.086 \\
OGLE-2013-SN-045 & 81.13370 & 20.446 & 0.088 \\
OGLE-2013-SN-045 & 85.65787 & 21.240 & 0.204 \\
OGLE-2013-SN-045 & 90.20165 & 20.832 & 0.166 \\
OGLE-2013-SN-045 & 92.94667 & 20.979 & 0.310 \\
OGLE-2013-SN-045 & 97.49925 & 21.071 & 0.246 \\
OGLE-2013-SN-045 & 102.94393 & 21.426 & 0.382 \\
OGLE-2013-SN-045 & 124.75345 & 20.945 & 0.208 \\
OGLE-2013-SN-045 & 146.50422 & 21.694 & 0.591 \\
\hline
OGLE-2013-SN-011 & 6.12206 & 19.526 & 0.039 \\
OGLE-2013-SN-011 & 11.83296 & 18.961 & 0.022 \\
OGLE-2013-SN-011 & 20.38365 & 18.915 & 0.028 \\
OGLE-2013-SN-011 & 25.11545 & 19.131 & 0.040 \\
OGLE-2013-SN-011 & 32.71402 & 18.973 & 0.020 \\
OGLE-2013-SN-011 & 41.29990 & 19.078 & 0.032 \\
OGLE-2013-SN-011 & 50.84806 & 19.136 & 0.042 \\
OGLE-2013-SN-011 & 52.72111 & 19.237 & 0.035 \\
OGLE-2013-SN-011 & 56.54574 & 19.224 & 0.033 \\
OGLE-2013-SN-011 & 61.27719 & 19.328 & 0.044 \\
OGLE-2013-SN-011 & 70.76037 & 19.283 & 0.035 \\
OGLE-2013-SN-011 & 78.35850 & 19.439 & 0.058 \\
OGLE-2013-SN-011 & 86.92428 & 19.780 & 0.062 \\
OGLE-2013-SN-011 & 93.54936 & 19.887 & 0.102 \\
OGLE-2013-SN-011 & 98.30835 & 20.117 & 0.108 \\
\hline
OGLE-2013-SN-005 & 2.65458 & 20.035 & 0.117 \\
OGLE-2013-SN-005 & 4.55711 & 19.814 & 0.054 \\
OGLE-2013-SN-005 & 8.33003 & 19.599 & 0.047 \\
OGLE-2013-SN-005 & 15.78589 & 19.574 & 0.062 \\
OGLE-2013-SN-005 & 27.89072 & 19.591 & 0.059 \\
OGLE-2013-SN-005 & 41.94150 & 19.588 & 0.069 \\
OGLE-2013-SN-005 & 58.74887 & 19.697 & 0.057 \\
OGLE-2013-SN-005 & 65.27442 & 19.958 & 0.120 \\
OGLE-2013-SN-005 & 71.81106 & 19.754 & 0.107 \\
OGLE-2013-SN-005 & 76.48508 & 19.971 & 0.089 \\
OGLE-2013-SN-005 & 209.52458 & 21.429 & 0.373 \\
\hline


==> data_OGLE_Ibandcalibrated_observerframe.tex <==
\hline
\hline
SN name & MJD & $I$ & $\Delta_I$ \\
\hline
OGLE-2014-SN-018 & 2456700.70108 & 99.999 & 9.999 \\
OGLE-2014-SN-018 & 2456703.71688 & 19.372 & 0.083 \\
OGLE-2014-SN-018 & 2456707.74095 & 18.589 & 0.022 \\
OGLE-2014-SN-018 & 2456710.70753 & 18.435 & 0.016 \\
OGLE-2014-SN-018 & 2456714.68800 & 18.437 & 0.025 \\
OGLE-2014-SN-018 & 2456728.67654 & 18.408 & 0.018 \\
OGLE-2014-SN-018 & 2456738.55525 & 18.328 & 0.017 \\
OGLE-2014-SN-018 & 2456742.57938 & 18.298 & 0.018 \\
OGLE-2014-SN-018 & 2456744.58520 & 18.306 & 0.018 \\
OGLE-2014-SN-018 & 2456745.55257 & 18.300 & 0.024 \\
OGLE-2014-SN-018 & 2456746.55567 & 18.417 & 0.029 \\
OGLE-2014-SN-018 & 2456747.53522 & 18.347 & 0.022 \\
OGLE-2014-SN-018 & 2456749.53478 & 18.305 & 0.019 \\
OGLE-2014-SN-018 & 2456793.45825 & 18.527 & 0.041 \\
OGLE-2014-SN-018 & 2456805.45459 & 19.099 & 0.065 \\
OGLE-2014-SN-018 & 2456889.91945 & 20.741 & 0.167 \\
\hline
OGLE-2014-SN-009 & 2456686.72316 & 99.999 & 9.999 \\
OGLE-2014-SN-009 & 2456689.72663 & 19.512 & 0.100 \\
OGLE-2014-SN-009 & 2456691.75320 & 19.355 & 0.079 \\
OGLE-2014-SN-009 & 2456692.75007 & 19.300 & 0.065 \\
OGLE-2014-SN-009 & 2456694.74193 & 19.079 & 0.049 \\
OGLE-2014-SN-009 & 2456697.73862 & 19.050 & 0.057 \\
OGLE-2014-SN-009 & 2456702.71556 & 19.072 & 0.073 \\
OGLE-2014-SN-009 & 2456706.70494 & 19.227 & 0.081 \\
OGLE-2014-SN-009 & 2456708.70683 & 19.190 & 0.061 \\
OGLE-2014-SN-009 & 2456711.69632 & 19.369 & 0.069 \\
OGLE-2014-SN-009 & 2456714.57626 & 19.372 & 0.096 \\
OGLE-2014-SN-009 & 2456717.64895 & 19.379 & 0.073 \\
OGLE-2014-SN-009 & 2456720.65968 & 19.451 & 0.080 \\
OGLE-2014-SN-009 & 2456723.66676 & 19.554 & 0.077 \\
OGLE-2014-SN-009 & 2456727.65855 & 19.447 & 0.076 \\
OGLE-2014-SN-009 & 2456731.65949 & 19.898 & 0.194 \\
OGLE-2014-SN-009 & 2456734.60567 & 19.618 & 0.102 \\
OGLE-2014-SN-009 & 2456738.61281 & 19.369 & 0.074 \\
OGLE-2014-SN-009 & 2456741.61426 & 19.846 & 0.099 \\
OGLE-2014-SN-009 & 2456742.58290 & 19.786 & 0.103 \\
OGLE-2014-SN-009 & 2456744.58868 & 19.491 & 0.095 \\
OGLE-2014-SN-009 & 2456745.55603 & 19.641 & 0.149 \\
OGLE-2014-SN-009 & 2456746.55913 & 19.712 & 0.138 \\
OGLE-2014-SN-009 & 2456747.53654 & 19.751 & 0.154 \\
OGLE-2014-SN-009 & 2456749.53607 & 19.663 & 0.112 \\
OGLE-2014-SN-009 & 2456753.54424 & 20.205 & 0.210 \\
OGLE-2014-SN-009 & 2456759.51941 & 20.021 & 0.160 \\
OGLE-2014-SN-009 & 2456763.50059 & 19.597 & 0.105 \\
OGLE-2014-SN-009 & 2456769.50642 & 20.020 & 0.131 \\
OGLE-2014-SN-009 & 2456772.50439 & 20.545 & 0.268 \\
OGLE-2014-SN-009 & 2456775.47257 & 20.284 & 0.204 \\
OGLE-2014-SN-009 & 2456793.46582 & 20.119 & 0.243 \\
OGLE-2014-SN-009 & 2456797.46251 & 21.049 & 0.607 \\
\hline
OGLE-2014-SN-004 & 2456657.78060 & 99.999 & 9.999 \\
OGLE-2014-SN-004 & 2456662.76829 & 18.725 & 0.040 \\
OGLE-2014-SN-004 & 2456668.74436 & 18.514 & 0.027 \\
OGLE-2014-SN-004 & 2456668.76158 & 18.527 & 0.026 \\
OGLE-2014-SN-004 & 2456673.75359 & 18.666 & 0.049 \\
OGLE-2014-SN-004 & 2456679.73902 & 18.653 & 0.025 \\
OGLE-2014-SN-004 & 2456692.67734 & 18.709 & 0.028 \\
OGLE-2014-SN-004 & 2456696.67355 & 18.693 & 0.030 \\
OGLE-2014-SN-004 & 2456700.65563 & 18.825 & 0.036 \\
OGLE-2014-SN-004 & 2456704.68576 & 18.633 & 0.043 \\
OGLE-2014-SN-004 & 2456709.53629 & 18.737 & 0.034 \\
OGLE-2014-SN-004 & 2456713.59979 & 18.718 & 0.045 \\
OGLE-2014-SN-004 & 2456735.59244 & 18.941 & 0.041 \\
OGLE-2014-SN-004 & 2456742.55684 & 19.089 & 0.048 \\
OGLE-2014-SN-004 & 2456743.56739 & 19.113 & 0.050 \\
OGLE-2014-SN-004 & 2456744.56266 & 19.139 & 0.053 \\
OGLE-2014-SN-004 & 2456745.52997 & 19.012 & 0.059 \\
OGLE-2014-SN-004 & 2456746.53312 & 19.069 & 0.076 \\
OGLE-2014-SN-004 & 2456749.49775 & 19.402 & 0.067 \\
OGLE-2014-SN-004 & 2456751.49432 & 19.654 & 0.080 \\
OGLE-2014-SN-004 & 2456752.55239 & 19.600 & 0.084 \\
OGLE-2014-SN-004 & 2456753.49694 & 19.779 & 0.116 \\
OGLE-2014-SN-004 & 2456754.48373 & 19.916 & 0.137 \\
OGLE-2014-SN-004 & 2456758.48356 & 21.612 & 0.646 \\
OGLE-2014-SN-004 & 2456759.47599 & 20.517 & 0.246 \\
OGLE-2014-SN-004 & 2456761.47847 & 20.821 & 0.293 \\
\hline
OGLE-2013-SN-144 & 2456629.73422 & 99.999 & 9.999 \\
OGLE-2013-SN-144 & 2456641.73318 & 18.490 & 0.020 \\
OGLE-2013-SN-144 & 2456647.74442 & 18.761 & 0.025 \\
OGLE-2013-SN-144 & 2456658.78541 & 18.829 & 0.018 \\
OGLE-2013-SN-144 & 2456661.81728 & 18.841 & 0.035 \\
OGLE-2013-SN-144 & 2456668.77739 & 18.950 & 0.025 \\
OGLE-2013-SN-144 & 2456675.76285 & 18.914 & 0.042 \\
OGLE-2013-SN-144 & 2456690.73007 & 19.102 & 0.028 \\
OGLE-2013-SN-144 & 2456695.68108 & 19.086 & 0.032 \\
OGLE-2013-SN-144 & 2456699.64183 & 19.190 & 0.040 \\
OGLE-2013-SN-144 & 2456704.69708 & 19.141 & 0.055 \\
OGLE-2013-SN-144 & 2456709.64793 & 19.391 & 0.042 \\
OGLE-2013-SN-144 & 2456713.62080 & 19.675 & 0.063 \\
OGLE-2013-SN-144 & 2456721.62124 & 19.784 & 0.054 \\
OGLE-2013-SN-144 & 2456742.56158 & 20.399 & 0.117 \\
OGLE-2013-SN-144 & 2456744.56742 & 21.222 & 0.273 \\
OGLE-2013-SN-144 & 2456745.53473 & 20.047 & 0.117 \\
OGLE-2013-SN-144 & 2456746.53785 & 20.959 & 0.287 \\
OGLE-2013-SN-144 & 2456749.50467 & 20.791 & 0.170 \\
\hline
OGLE-2013-SN-135 & 2456618.64749 & 99.999 & 9.999 \\
OGLE-2013-SN-135 & 2456622.67044 & 19.726 & 0.083 \\
OGLE-2013-SN-135 & 2456633.62744 & 18.970 & 0.053 \\
OGLE-2013-SN-135 & 2456636.60643 & 18.779 & 0.040 \\
OGLE-2013-SN-135 & 2456638.62247 & 18.744 & 0.036 \\
OGLE-2013-SN-135 & 2456640.62224 & 18.967 & 0.056 \\
OGLE-2013-SN-135 & 2456644.62094 & 18.943 & 0.055 \\
OGLE-2013-SN-135 & 2456646.61001 & 18.867 & 0.045 \\
OGLE-2013-SN-135 & 2456649.64924 & 18.949 & 0.051 \\
OGLE-2013-SN-135 & 2456651.59131 & 19.006 & 0.048 \\
OGLE-2013-SN-135 & 2456654.60400 & 18.908 & 0.041 \\
OGLE-2013-SN-135 & 2456656.57083 & 18.965 & 0.040 \\
OGLE-2013-SN-135 & 2456658.61392 & 19.046 & 0.047 \\
OGLE-2013-SN-135 & 2456659.59563 & 19.010 & 0.051 \\
OGLE-2013-SN-135 & 2456662.60705 & 18.977 & 0.042 \\
OGLE-2013-SN-135 & 2456664.64610 & 18.861 & 0.038 \\
OGLE-2013-SN-135 & 2456667.63458 & 18.970 & 0.057 \\
OGLE-2013-SN-135 & 2456669.59803 & 18.849 & 0.047 \\
OGLE-2013-SN-135 & 2456672.58228 & 18.834 & 0.071 \\
OGLE-2013-SN-135 & 2456675.57229 & 18.994 & 0.083 \\
OGLE-2013-SN-135 & 2456677.59701 & 18.825 & 0.040 \\
OGLE-2013-SN-135 & 2456679.59276 & 18.989 & 0.036 \\
OGLE-2013-SN-135 & 2456687.61965 & 19.116 & 0.050 \\
OGLE-2013-SN-135 & 2456689.58419 & 19.063 & 0.048 \\
OGLE-2013-SN-135 & 2456691.53336 & 20.244 & 0.167 \\
OGLE-2013-SN-135 & 2456694.57958 & 19.070 & 0.053 \\
OGLE-2013-SN-135 & 2456696.53032 & 19.104 & 0.062 \\
OGLE-2013-SN-135 & 2456698.61169 & 18.938 & 0.048 \\
OGLE-2013-SN-135 & 2456701.53245 & 19.132 & 0.065 \\
OGLE-2013-SN-135 & 2456704.57621 & 18.893 & 0.057 \\
OGLE-2013-SN-135 & 2456706.58618 & 19.116 & 0.057 \\
OGLE-2013-SN-135 & 2456709.54774 & 19.270 & 0.059 \\
OGLE-2013-SN-135 & 2456711.57484 & 19.034 & 0.053 \\
OGLE-2013-SN-135 & 2456714.52181 & 19.276 & 0.094 \\
OGLE-2013-SN-135 & 2456720.54212 & 19.091 & 0.063 \\
OGLE-2013-SN-135 & 2456726.57680 & 19.379 & 0.069 \\
OGLE-2013-SN-135 & 2456728.52057 & 19.603 & 0.103 \\
OGLE-2013-SN-135 & 2456731.54330 & 19.706 & 0.146 \\
OGLE-2013-SN-135 & 2456734.51610 & 19.464 & 0.102 \\
OGLE-2013-SN-135 & 2456738.50884 & 19.626 & 0.088 \\
OGLE-2013-SN-135 & 2456742.49394 & 19.861 & 0.156 \\
OGLE-2013-SN-135 & 2456744.48566 & 20.400 & 0.264 \\
\hline
OGLE-2013-SN-048 & 2456487.91564 & 99.999 & 9.999 \\
OGLE-2013-SN-048 & 2456490.93478 & 20.955 & 0.221 \\
OGLE-2013-SN-048 & 2456496.89943 & 20.010 & 0.164 \\
OGLE-2013-SN-048 & 2456498.89241 & 20.095 & 0.138 \\
OGLE-2013-SN-048 & 2456508.84070 & 19.654 & 0.078 \\
OGLE-2013-SN-048 & 2456515.83033 & 19.630 & 0.051 \\
OGLE-2013-SN-048 & 2456519.75978 & 19.752 & 0.064 \\
OGLE-2013-SN-048 & 2456522.75844 & 19.612 & 0.070 \\
OGLE-2013-SN-048 & 2456525.76699 & 19.865 & 0.131 \\
OGLE-2013-SN-048 & 2456532.81934 & 19.745 & 0.081 \\
OGLE-2013-SN-048 & 2456534.87731 & 19.633 & 0.059 \\
OGLE-2013-SN-048 & 2456543.83559 & 19.665 & 0.063 \\
OGLE-2013-SN-048 & 2456546.76863 & 19.636 & 0.049 \\
OGLE-2013-SN-048 & 2456548.72912 & 19.573 & 0.052 \\
OGLE-2013-SN-048 & 2456552.66567 & 19.426 & 0.099 \\
OGLE-2013-SN-048 & 2456555.70276 & 19.558 & 0.087 \\
OGLE-2013-SN-048 & 2456559.67595 & 19.713 & 0.071 \\
OGLE-2013-SN-048 & 2456562.71309 & 19.752 & 0.059 \\
OGLE-2013-SN-048 & 2456565.71028 & 19.648 & 0.050 \\
OGLE-2013-SN-048 & 2456571.68499 & 19.820 & 0.071 \\
OGLE-2013-SN-048 & 2456576.71394 & 19.815 & 0.059 \\
OGLE-2013-SN-048 & 2456581.68987 & 19.879 & 0.101 \\
OGLE-2013-SN-048 & 2456585.70248 & 20.121 & 0.129 \\
OGLE-2013-SN-048 & 2456590.61244 & 19.951 & 0.122 \\
OGLE-2013-SN-048 & 2456595.58447 & 19.911 & 0.080 \\
OGLE-2013-SN-048 & 2456603.62601 & 19.957 & 0.096 \\
OGLE-2013-SN-048 & 2456609.59866 & 20.519 & 0.182 \\
OGLE-2013-SN-048 & 2456614.66305 & 20.667 & 0.216 \\
OGLE-2013-SN-048 & 2456618.59640 & 20.558 & 0.162 \\
OGLE-2013-SN-048 & 2456633.59524 & 21.483 & 0.453 \\
OGLE-2013-SN-048 & 2456638.60189 & 21.566 & 0.446 \\
\hline
OGLE-2013-SN-047 & 2456500.84177 & 99.999 & 9.999 \\
OGLE-2013-SN-047 & 2456509.82132 & 18.245 & 0.017 \\
OGLE-2013-SN-047 & 2456515.81102 & 18.145 & 0.015 \\
OGLE-2013-SN-047 & 2456518.88063 & 18.195 & 0.017 \\
OGLE-2013-SN-047 & 2456521.65666 & 18.281 & 0.019 \\
OGLE-2013-SN-047 & 2456524.76042 & 18.308 & 0.023 \\
OGLE-2013-SN-047 & 2456531.80594 & 18.526 & 0.025 \\
OGLE-2013-SN-047 & 2456534.82196 & 18.582 & 0.022 \\
OGLE-2013-SN-047 & 2456538.76709 & 18.671 & 0.028 \\
OGLE-2013-SN-047 & 2456546.68962 & 18.749 & 0.022 \\
OGLE-2013-SN-047 & 2456548.59075 & 18.834 & 0.033 \\
OGLE-2013-SN-047 & 2456553.81399 & 18.720 & 0.052 \\
OGLE-2013-SN-047 & 2456558.72850 & 18.828 & 0.028 \\
OGLE-2013-SN-047 & 2456561.69262 & 18.971 & 0.028 \\
OGLE-2013-SN-047 & 2456564.66533 & 18.933 & 0.027 \\
OGLE-2013-SN-047 & 2456568.66325 & 18.989 & 0.027 \\
OGLE-2013-SN-047 & 2456572.64707 & 19.063 & 0.030 \\
OGLE-2013-SN-047 & 2456577.62366 & 19.168 & 0.037 \\
OGLE-2013-SN-047 & 2456582.62181 & 19.142 & 0.040 \\
OGLE-2013-SN-047 & 2456585.64134 & 19.335 & 0.077 \\
OGLE-2013-SN-047 & 2456590.64918 & 19.675 & 0.077 \\
OGLE-2013-SN-047 & 2456592.65724 & 19.992 & 0.075 \\
OGLE-2013-SN-047 & 2456596.63832 & 20.538 & 0.185 \\
OGLE-2013-SN-047 & 2456602.53295 & 20.341 & 0.136 \\
OGLE-2013-SN-047 & 2456608.53420 & 20.392 & 0.123 \\
OGLE-2013-SN-047 & 2456611.56742 & 20.339 & 0.150 \\
OGLE-2013-SN-047 & 2456614.53614 & 21.172 & 0.372 \\
OGLE-2013-SN-047 & 2456620.62880 & 20.833 & 0.197 \\
OGLE-2013-SN-047 & 2456624.57273 & 20.674 & 0.168 \\
OGLE-2013-SN-047 & 2456625.55033 & 20.612 & 0.188 \\
OGLE-2013-SN-047 & 2456630.54591 & 21.106 & 0.326 \\
OGLE-2013-SN-047 & 2456631.55025 & 20.950 & 0.196 \\
OGLE-2013-SN-047 & 2456637.55074 & 20.970 & 0.305 \\
OGLE-2013-SN-047 & 2456644.55464 & 21.278 & 0.430 \\
OGLE-2013-SN-047 & 2456650.58556 & 21.491 & 0.361 \\
OGLE-2013-SN-047 & 2456657.53278 & 21.293 & 0.466 \\
OGLE-2013-SN-047 & 2456664.57720 & 21.247 & 0.282 \\
\hline
OGLE-2013-SN-046 & 2456487.89680 & 99.999 & 9.999 \\
OGLE-2013-SN-046 & 2456491.88230 & 19.794 & 0.071 \\
OGLE-2013-SN-046 & 2456497.94554 & 19.455 & 0.131 \\
OGLE-2013-SN-046 & 2456498.92569 & 19.446 & 0.064 \\
OGLE-2013-SN-046 & 2456508.82159 & 19.662 & 0.059 \\
OGLE-2013-SN-046 & 2456514.80302 & 19.543 & 0.049 \\
OGLE-2013-SN-046 & 2456517.84941 & 19.670 & 0.091 \\
OGLE-2013-SN-046 & 2456521.73948 & 19.652 & 0.064 \\
OGLE-2013-SN-046 & 2456524.81792 & 19.712 & 0.074 \\
OGLE-2013-SN-046 & 2456530.83411 & 19.626 & 0.060 \\
OGLE-2013-SN-046 & 2456533.81872 & 19.618 & 0.047 \\
OGLE-2013-SN-046 & 2456539.89338 & 19.855 & 0.067 \\
OGLE-2013-SN-046 & 2456545.76713 & 19.622 & 0.039 \\
OGLE-2013-SN-046 & 2456547.71357 & 19.706 & 0.067 \\
OGLE-2013-SN-046 & 2456569.71884 & 19.940 & 0.053 \\
OGLE-2013-SN-046 & 2456573.72469 & 20.105 & 0.066 \\
OGLE-2013-SN-046 & 2456578.66547 & 20.099 & 0.077 \\
OGLE-2013-SN-046 & 2456589.67142 & 20.717 & 0.182 \\
OGLE-2013-SN-046 & 2456600.60743 & 20.747 & 0.150 \\
OGLE-2013-SN-046 & 2456602.59129 & 21.007 & 0.184 \\
OGLE-2013-SN-046 & 2456603.56146 & 20.845 & 0.188 \\
OGLE-2013-SN-046 & 2456605.65176 & 21.561 & 0.388 \\
OGLE-2013-SN-046 & 2456610.59287 & 20.904 & 0.226 \\
OGLE-2013-SN-046 & 2456613.60076 & 21.693 & 0.485 \\
OGLE-2013-SN-046 & 2456622.56807 & 21.575 & 0.279 \\
OGLE-2013-SN-045 & 2456480.86619 & 99.999 & 9.999 \\
OGLE-2013-SN-045 & 2456485.86382 & 19.961 & 0.059 \\
OGLE-2013-SN-045 & 2456490.86248 & 20.152 & 0.097 \\
OGLE-2013-SN-045 & 2456494.71104 & 20.159 & 0.191 \\
OGLE-2013-SN-045 & 2456500.84177 & 19.913 & 0.112 \\
OGLE-2013-SN-045 & 2456509.82132 & 19.832 & 0.060 \\
OGLE-2013-SN-045 & 2456515.81102 & 19.825 & 0.058 \\
OGLE-2013-SN-045 & 2456518.88063 & 19.942 & 0.067 \\
OGLE-2013-SN-045 & 2456521.65666 & 19.950 & 0.075 \\
OGLE-2013-SN-045 & 2456524.76042 & 20.057 & 0.107 \\
OGLE-2013-SN-045 & 2456531.80594 & 20.005 & 0.084 \\
OGLE-2013-SN-045 & 2456534.82196 & 20.025 & 0.070 \\
OGLE-2013-SN-045 & 2456538.76709 & 20.251 & 0.108 \\
OGLE-2013-SN-045 & 2456546.68962 & 20.417 & 0.093 \\
OGLE-2013-SN-045 & 2456548.59075 & 20.111 & 0.096 \\
OGLE-2013-SN-045 & 2456553.81399 & 20.254 & 0.203 \\
OGLE-2013-SN-045 & 2456558.72850 & 20.096 & 0.080 \\
OGLE-2013-SN-045 & 2456561.69262 & 20.304 & 0.083 \\
OGLE-2013-SN-045 & 2456564.66533 & 20.232 & 0.076 \\
OGLE-2013-SN-045 & 2456568.66325 & 20.453 & 0.086 \\
OGLE-2013-SN-045 & 2456572.64707 & 20.344 & 0.088 \\
OGLE-2013-SN-045 & 2456577.62366 & 21.146 & 0.204 \\
OGLE-2013-SN-045 & 2456582.62181 & 20.745 & 0.166 \\
OGLE-2013-SN-045 & 2456585.64134 & 20.896 & 0.310 \\
OGLE-2013-SN-045 & 2456590.64918 & 20.996 & 0.246 \\
OGLE-2013-SN-045 & 2456596.63832 & 21.359 & 0.382 \\
OGLE-2013-SN-045 & 2456620.62880 & 20.901 & 0.208 \\
OGLE-2013-SN-045 & 2456644.55464 & 21.650 & 0.591 \\
\hline
OGLE-2013-SN-011 & 2456291.79407 & 99.999 & 9.999 \\
OGLE-2013-SN-011 & 2456304.67816 & 19.421 & 0.039 \\
OGLE-2013-SN-011 & 2456310.67461 & 18.863 & 0.022 \\
OGLE-2013-SN-011 & 2456319.65283 & 18.827 & 0.028 \\
OGLE-2013-SN-011 & 2456324.62122 & 19.048 & 0.040 \\
OGLE-2013-SN-011 & 2456332.59972 & 18.899 & 0.020 \\
OGLE-2013-SN-011 & 2456341.61489 & 19.013 & 0.032 \\
OGLE-2013-SN-011 & 2456351.64046 & 19.080 & 0.042 \\
OGLE-2013-SN-011 & 2456353.60717 & 19.183 & 0.035 \\
OGLE-2013-SN-011 & 2456357.62303 & 19.174 & 0.033 \\
OGLE-2013-SN-011 & 2456362.59105 & 19.283 & 0.044 \\
OGLE-2013-SN-011 & 2456372.54839 & 19.246 & 0.035 \\
OGLE-2013-SN-011 & 2456380.52643 & 19.409 & 0.058 \\
OGLE-2013-SN-011 & 2456389.52049 & 19.757 & 0.062 \\
OGLE-2013-SN-011 & 2456396.47683 & 19.869 & 0.102 \\
OGLE-2013-SN-011 & 2456401.47377 & 20.103 & 0.108 \\
\hline
OGLE-2013-SN-005 & 2456238.71155 & 99.999 & 9.999 \\
OGLE-2013-SN-005 & 2456244.54040 & 19.864 & 0.117 \\
OGLE-2013-SN-005 & 2456246.57611 & 19.647 & 0.054 \\
OGLE-2013-SN-005 & 2456250.61313 & 19.438 & 0.047 \\
OGLE-2013-SN-005 & 2456258.59090 & 19.425 & 0.062 \\
OGLE-2013-SN-005 & 2456271.54307 & 19.461 & 0.059 \\
OGLE-2013-SN-005 & 2456286.57740 & 19.479 & 0.069 \\
OGLE-2013-SN-005 & 2456304.56129 & 19.612 & 0.057 \\
OGLE-2013-SN-005 & 2456311.54363 & 19.881 & 0.120 \\
OGLE-2013-SN-005 & 2456318.53783 & 19.685 & 0.107 \\
OGLE-2013-SN-005 & 2456323.53904 & 19.908 & 0.089 \\
OGLE-2013-SN-005 & 2456465.89130 & 21.412 & 0.373 \\
\hline

==> table_info.tex <==
\hline
SN name & $z_\mathrm{host}$ & $\mu$ (mag) & E(B-V)$_\mathrm{MW}$ & Explosion (MJD) \\
\hline
OGLE-2014-SN-018 & 0.03 & 35.56 & 0.087 & 2456702.2 $\pm$ 1.5 \\
OGLE-2014-SN-009 & 0.056 & 36.96 & 0.068 & 2456688.2 $\pm$ 1.5 \\
OGLE-2014-SN-004 & 0.03 & 35.56 & 0.067 & 2456660.3 $\pm$ 2.5 \\
OGLE-2013-SN-144 & 0.04 & 36.21 & 0.113 & 2456635.7 $\pm$ 6.0 \\
OGLE-2013-SN-135 & 0.057 & 37.00 & 0.157 & 2456620.65 $\pm$ 2.05 \\
OGLE-2013-SN-048 & 0.06 & 37.12 & 0.038 & 2456489.4 $\pm$ 1.5 \\
OGLE-2013-SN-047 & 0.06 & 37.12 & 0.029 & 2456505.3 $\pm$ 4.5 \\
OGLE-2013-SN-046 & 0.07 & 37.47 & 0.028 & 2456489.9 $\pm$ 2.0 \\
OGLE-2013-SN-045 & 0.10 & 38.29 & 0.030 & 2456483.4 $\pm$ 2.5 \\
OGLE-2013-SN-011 & 0.05 & 36.71 & 0.047 & 2456298.25 $\pm$ 6.45 \\
OGLE-2013-SN-005 & 0.07 & 37.47 & 0.028 & 2456241.7 $\pm$ 2.9 \\
\hline

